Influence Paths for Characterizing Subject-Verb Number Agreement in LSTM Language Models

LSTM-based recurrent neural networks are the state-of-the-art for many natural language processing (NLP) tasks. Despite their performance, it is unclear whether, or how, LSTMs learn structural features of natural languages such as subject-verb number agreement in English. Lacking this understanding, the generality of LSTM performance on this task and their suitability for related tasks remains uncertain. Further, errors cannot be properly attributed to a lack of structural capability, training data omissions, or other exceptional faults. We introduce *influence paths*, a causal account of structural properties as carried by paths across gates and neurons of a recurrent neural network. The approach refines the notion of influence (the subject's grammatical number has influence on the grammatical number of the subsequent verb) into a set of gate or neuron-level paths. The set localizes and segments the concept (e.g., subject-verb agreement), its constituent elements (e.g., the subject), and related or interfering elements (e.g., attractors). We exemplify the methodology on a widely-studied multi-layer LSTM language model, demonstrating its accounting for subject-verb number agreement. The results offer both a finer and a more complete view of an LSTM's handling of this structural aspect of the English language than prior results based on diagnostic classifiers and ablation.

==> Makefile <==
OS   := $(shell uname)
ifeq ($(OS), Linux)
  OPEN := evince
else
ifneq ("$(wildcard /Applications/Skim.app)","")
  OPEN := open -a /Applications/Skim.app
else
  OPEN := open -a /Applications/Preview.app
endif
endif
DOC  := doc-rnn-influence-pathways
MAIN := preamble
PDFLATEX := pdflatex

DEP_FIGS := $(shell find ./figures \
	-name '*.tex' \
	)
DEP := *.tex *.bib $(DEP_FIGS)
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))

start:
	make draft

start-%:
	make open-$*
	make watch-$*

draft:
	make start-draft

final:
	make start-final

$(DOC).final.main.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 1-9 output $@

$(DOC).final.supplemental.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 10-12 output $@

parts: $(DOC).final.main.pdf $(DOC).final.supplemental.pdf

startt:
	$(PDFLATEX) $(QUIET) preamble; $(BIBTEX) $(QUIET) $(MAIN); $(PDFLATEX) $(QUIET) preamble; $(PDFLATEX) $(QUIET) preamble;
	make clean; $(OPEN) preamble.pdf

open-%: $(DOC).%.pdf
ifneq ("$(OPEN)","")
	$(OPEN) $(DOC).$*.pdf ; sleep 1
else
	@echo "Could not find a PDF reader. If you'd like this \
	makefile to open the generated pdfs, add your PDF reader to \
	the opening section of the Makefile."
	@exit 1
endif

$(DOC).pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).pdf
	@cp $(MAIN).synctex.gz $(DOC).synctex.gz


$(DOC).%.pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\def\$*{}\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).$*.pdf
	@cp $(MAIN).synctex.gz $(DOC).$*.synctex.gz

watch-%:
	perl watch.pl watch $(DOC).$*.pdf $(DEP)
	perl watch.pl watch $(DOC).pdf $(DEP)

# DEBUGGING UTILS
# https://www.cmcrossroads.com/article/printing-value-makefile-variable
print-%  : ; @echo $* = $($*)

debug: $(DEP)
	$(PDFLATEX) -interaction nonstopmode "\input{$(MAIN).tex}"
	$(OPEN) $(DOC).pdf

# To debug unicode issues:
# useful emacs command: find-file-literally
show_unicode: $(DEP)
	pcregrep --color='auto' -n "[\x80-\xFF]" *.tex *.bib

# List all references to the thing after find_ in the tex sources.
find_%: *.tex
	grep -I -C 1 -n --color=auto '$*' *.tex; true

# CLEANING
clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.run.xml; true
	rm -Rf *~; true
	rm -Rf $(DOC).pdf $(MAIN).pdf $(DOC).*.pdf; true
	rm -Rf main-blx.bib
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true

desvn:
	find . -type d -name .svn -exec rm -rf {} +

#ARTIFACTS := $(shell find artifact)

#artifact: ${ARTIFACTS}
#	COPYFILE_DISABLE=1 tar -cvf artifact.tar artifact
#	gzip artifact.tar

# PACKAGING

DEP_TEX := $(shell find . \
	-not \( -path ./old-sections -prune \) \
	-not \( -path ./supplemental -prune \) \
	-not \( -path ./ijcai2018-formatting-guidelines -prune \) \
	-not \( -path ./arXiv -prune \) \
	-not \( -path ./formatting_instructions -prune \) \
	-not \( -path ./styles -prune \) \
	-name '*.tex' \
	)

DEP_TEX2 := $(DEP_TEX:%=arXiv/%)

arXiv/%.tex: %.tex
	latexpand --empty-comments $< > arXiv/$<
	sed -e '/^\s*%/d' -i '' arXiv/$<

arXiv:
	mkdir arXiv
	mkdir arXiv/figures

$(MAIN).bbl: $(DOC).arXiv.pdf

bundle: $(MAIN).bbl arXiv $(DEP_TEX:%=arXiv/%) ijcai18.sty
	cp -R $(MAIN).bbl ijcai18.sty arXiv
	cp -R $(DEP_FIGS) arXiv/figures
	(echo "\def\\\\arXiv{}\n"; cat arXiv/$(MAIN).tex) \
           > arXiv/$(MAIN).tex.temp
	mv arXiv/$(MAIN).tex.temp arXiv/$(MAIN).tex
	tar -cvf arXiv.tar arXiv
	gzip arXiv.tar

rebundle:
	rm -Rf arXiv; true
	rm -Rf arXiv.tar.gz; true
	make bundle


==> figures/fig-lstm.tex <==
%\documentclass[tikz]{standalone}

%\usepackage{tikz}
%\usetikzlibrary{arrows,shapes,backgrounds,fit,positioning}
%\graphicspath{{images/}}

%\input{defs}
%\input{commenting}

%\begin{document}

\def\first{-2}
\def\last{2}

\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}

\newcommand{\tsub}[1]{
  \ifthenelse{#1 < 0}{
    t#1
  }{
    \ifthenelse{#1 = 0}{
      t
    }{
      t+#1
    }
  }
}

\newcommand{\showmid}[1]{
  \ifthenelse{\t > \first \and \t < \last}{
    #1
  }{

  }
}

\begin{tikzpicture}[
  every node/.style={%
    inner sep=2pt,
    font=\small,
  }
  ]

  \tikzstyle{ctime} = [draw=black,line width=1.0pt,>=latex]
  \tikzstyle{ptime} = [draw=gray,line width=1.0pt,>=latex]

  \foreach \t in {\first,...,\last} {
    \pgfmathsetmacro\pt{\t-1};
    \pgfmathsetmacro\nt{\t+1};

    % input X_t
    \node[] at (3.5*\t,+1) (input\t) {\showmid{$X_{\tsub{\t}}$}};
    \coordinate (midinput\t) at ([xshift=-1.5cm,yshift=-0.5cm]input\t);

    % combination in/forget
    \node[below of=input\t] (inforget\t) {\showmid{$f_{\tsub{\t}}$ $i_{\tsub{\t}}$}};

    % cell state c_t,
    \node[below of=inforget\t] (precell\t) {\showmid{$\tilde{c}_{\tsub{\t}}$}};
    \node[below of=precell\t] (cell\t) {\showmid{$c_{\tsub{\t}}$}};

    % output o_t, % not output of model
    \node[below of=cell\t] (out\t) {\showmid{$o_{\tsub{\t}}$}};

    % hidden h_t,
    \node[below of=out\t] (hidden\t) {\showmid{$h_{\tsub{\t}}$}};

    % output of model E_t
    \node[below of=hidden\t] (output\t) {\showmid{$E_{\tsub{\t}}$}};
    \coordinate (midhidden\t) at ([xshift=1.25cm,yshift=0.5cm]hidden\t);

    % lstm block
    \begin{scope}[on background layer]
      \ifthen{\t > \first \and \t < \last}{
        \node[minimum width=2cm,fit=(inforget\t)(cell\t)(out\t)(hidden\t),rounded corners,fill=gray!25] {};
      }
    \end{scope}

    \ifthen{\t > \first \and \t < \last}{
      \draw[ctime,rounded corners] (input\t) -| (midinput\t);
      \draw[ctime,->,rounded corners] (midinput\t) |- ([yshift=0.25cm]inforget\t);
      \draw[ctime,->,rounded corners] (midinput\t) |- ([yshift=0.5cm]precell\t);
      \draw[ctime,->,rounded corners] (midinput\t) |- ([yshift=0.5cm]out\t);

      \draw[ctime,->] (precell\t) -- (cell\t);
      \draw[ctime,->] (out\t) -- (hidden\t);
      \draw[ctime,->] (cell\t) edge[bend left=45] (hidden\t);
      \draw[ctime,->] (hidden\t) -- (output\t);

      \draw[ctime,->] (inforget\t) edge[bend left=45] ([yshift=0.5cm]cell\t); % from in
    }
  }

  \foreach \t in {\first,...,\last} {
    \pgfmathsetmacro\pt{\t-1};
    \pgfmathsetmacro\nt{\t+1};

    \pgfmathsetmacro\firstplusone{\first+1};
    \ifthen{\t = \firstplusone}{
      \draw[dashed,ptime] (cell\pt) -- ([xshift=-1cm]cell\pt);
      \draw[dashed,ptime] (hidden\pt) -- ([xshift=-1cm]hidden\pt);
    }

    \ifthenelse{\t > \first}{
      \ifthenelse{\t < \last}{
        \draw[ptime,->] (cell\pt) -- (cell\t);
        \draw[ptime,rounded corners] (hidden\pt) -| (midhidden\pt);
        \draw[ptime,->,rounded corners] (midhidden\pt) |- ([yshift=-0.5cm]inforget\t);
        \draw[ptime,->,rounded corners] (midhidden\pt) |- ([yshift=-0.5cm]precell\t);
        \draw[ptime,->,rounded corners] (midhidden\pt) |- ([yshift=-0.5cm]out\t);
        \draw[ctime,->] (inforget\t) edge[bend left=-45] ([xshift=-1.0cm]cell\t); % from forget
      }{
        \draw[ptime,rounded corners] (hidden\pt) -- ([xshift=1cm]hidden\pt);
        \draw[dashed,ptime] ([xshift=1cm]hidden\pt) -- ([xshift=2cm]hidden\pt);
        \draw[ptime] (cell\pt) -- ([xshift=1cm]cell\pt);
        \draw[dashed,ptime] ([xshift=1cm]cell\pt) -- ([xshift=2cm]cell\pt);
      }
    }
  }
\end{tikzpicture}

%\end{document}

